LCP: A Low-Communication Parallelization Method for Fast Neural Network Inference in Image Recognition

Deep neural networks (DNNs) have inspired new studies in myriad edge applications with robots, autonomous agents, and Internet-of-things (IoT) devices. However, performing inference of DNNs in the edge is still a severe challenge, mainly because of the contradiction between the intensive resource requirements of DNNs and the tight resource availability in several edge domains. Further, as communication is costly, taking advantage of other available edge devices by using data- or model-parallelism methods is not an effective solution. To benefit from available compute resources with low communication overhead, we propose the first DNN parallelization method for reducing the communication overhead in a distributed system. We propose a low-communication parallelization (LCP) method in which models consist of several almost-independent and narrow branches. LCP offers close-to-minimum communication overhead with better distribution and parallelization opportunities while significantly reducing memory footprint and computation compared to data- and model-parallelism methods. We deploy LCP models on three distributed systems: AWS instances, Raspberry Pis, and PYNQ boards. We also evaluate the performance of LCP models on a customized hardware (tailored for low latency) implemented on a small edge FPGA and as a 16mW 0.107mm2 ASIC @7nm chip. LCP models achieve a maximum and average speedups of 56x and 7x, compared to the originals, which could be improved by up to an average speedup of 33x by incorporating common optimizations such as pruning and quantization.

==> tex/table-common-vision-corl.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%

\renewcommand{\arraystretch}{0.88}
\begin{table}[t]
\scriptsize
\vspace{0pt}
\centering
\caption{Results of split-only DNN models on MNIST, Cifar10/100, and Flower102 datasets. fc: fully-connected, c: convolution, p: pooling, n: normalization, and d: dropout.}
\vspace{5pt}
\adjustbox{max width=0.9\textwidth}{
\begin{tabular}{c || c | c | c | c | c | c | c | c  }
  \toprule
   \multirow{2}{*}{\textbf{Model Name}} 
      & \multirow{2}{*}{\textbf{Dataset}}
      & \multirow{2}{*}{\textbf{Classes}}
      & \textbf{Input}
      & \multirow{2}{*}{\textbf{Branches}}
      & {\textbf{Top-1}}
      & {\textbf{Top-5}}
      & \textbf{Number of} 
      & \textbf{Number of} \\
   
            
      & 
      &
      & \textbf{Size}
      &
      & {\textbf{Accuracy}}
      & {\textbf{Accuracy}}
      & \textbf{Parameters}
      & \textbf{MAC Operations}\\
  \midrule 
  
    %  \textbf{LeNet-FC}
     
    %  & \textbf{MNIST} 
    %  & \textbf{10}
    %  & \textbf{28$\x$28}  
    %  & \textbf{1} 
    %  & \textbf{97.95}
    %  & \textbf{99.97}
    %  & \textbf{266.6k}
    %  & \textbf{266.2k}
     
    %  \\    
    %  LeNet-FC-split2
     
    %  & MNIST
    %  & 10
    %  & 28$\x$28    
    %  & 2 
    %  & 98.20
    %  & 99.99
    %  & 134.0k
    %  & 134.1k
     
    %  \\     
    %  LeNet-FC-split4
     
    %  & MNIST
    %  & 10 
    %  & 28$\x$28   
    %  & 4 
    %  & 97.84
    %  & 99.98
    %  & 67.7k
    %  & 67.1k
     
    %  \\
    %  LeNet-FC-split8
     
    %  & MNIST 
    %  & 10
    %  & 28$\x$28   
    %  & 8 
    %  & 97.05
    %  & 99.95
    %  & 33.9k
    %  & 33.8k
     
    %  \\
    %  \midrule
    %  %-------------------------------------------
      \textbf{LeNet}
      
      & \textbf{MNIST}
      & \textbf{10}
      & \textbf{28$\x$28}   
      & \textbf{1} 
      & \textbf{98.76}  
      & \textbf{99.97}
      & \textbf{61.7k}
      & \textbf{61.5k}
      \\
      
      LeNet-split2 
      & MNIST
      & 10 
      & 28$\x$28   
      & 2 
      & 98.86 
      & 99.99
      & 31.5k
      & 30.5k 
      \\
      
      LeNet-split4 
      & MNIST
      & 10 
      & 28$\x$28   
      & 4
      & 98.93 
      & 99.98
      & 16.1k
      & 16.0k 
      \\
      
      LeNet-split8 
      & MNIST
      & 10 
      & 28$\x$28    
      & 8
      & 98.81
      & 99.98
      & 8.8k
      & 8.5k
      \\
      
      \midrule
     %-------------------------------------------
     \textbf{CifarNet}
     
     & \textbf{Cifar10} 
     & \textbf{10}
     & \textbf{32$\x$32}    
     & \textbf{1}
     & \textbf{83.41}
     & \textbf{98.86}
     & \textbf{797.97k}
     & \textbf{14.79M}
     
     \\
     CifarNet-split2
     
     & Cifar10
     & 10 
     & 32$\x$32  
     & 2
     & 80.63 
     & 98.80
     & 401.75k
     & 9.32M
     
     \\
     CifarNet-split4
     
     & Cifar10
     & 10
     & 32$\x$32  
     & 4 
     & 79.53
     & 98.80
     & 203.64k
     & 6.59M
     
     \\
     CifarNet-split8
     
     & Cifar10
     & 10  
     & 32$\x$32  
     & 8
     & 76.70
     & 98.40
     & 104.6k
     & 5.22M
     
     
     \\
     \midrule
     
     %-------------------------------------------
     \textbf{CifarNet}
     
     & \textbf{Cifar100} 
     & \textbf{100}
     & \textbf{32$\x$32}    
     & \textbf{1}
     & \textbf{52.87}
     & \textbf{80.97}
     & \textbf{815.34k}
     & \textbf{14.81M}
     
     \\
     CifarNet-split2
     
     & Cifar100
     & 100
     & 32$\x$32  
     & 2
     & 51.22
     & 79.80
     & 410.48k
     & 9.33M
     
     \\
     CifarNet-split4
     
     & Cifar100
     & 100
     & 32$\x$32  
     & 4 
     & 48.48
     & 78.22
     & 208.05k
     & 6.59M
     
     \\
     CifarNet-split8
     
     & Cifar100
     & 100  
     & 32$\x$32  
     & 8
     & 47.98
     & 76.86
     & 106.85k
     & 5.23M
     
     
     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Cifar100}
     & \textbf{100}
     & \textbf{32$\x$32}  
     & \textbf{1}
     & \textbf{50.33}
     & \textbf{75.26}
     & \textbf{76.15M}
     & \textbf{154.09M}
     
     \\
     VGG-S-split2
     
     & Cifar100  
     & 100
     & 32$\x$32 
     & 2
     & 48.53  
     & 75.33
     & 38.09M
     & 78.28M
     
     \\
     VGG-S-split4
     
     & Cifar100
     & 100
     & 32$\x$32 
     & 4
     & 47.72    
     & 76.70
     & 19.06M
     & 40.37M
     
     \\
     VGG-S-split8
     
     & Cifar100
     & 100 
     & 32$\x$32   
     & 8 
     & 48.48
     & 77.66
     & 9.54M
     & 21.42M

     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Flower102}
     & \textbf{102}  
     & \textbf{224$\x$224}  
     & \textbf{1}
     & \textbf{88.14}
     & \textbf{97.02}
     & \textbf{60.79M}
     & \textbf{1.85G}
     
     \\
     VGG-S-split2
     
     & Flower102  
     & 102
     & 224$\x$224 
     & 2
     & 89.31  
     & 97.77
     & 30.50M
     & 1.01G
     
     \\
     VGG-S-split4
     
     & Flower102
     & 102 
     & 224$\x$224 
     & 4
     & 87.55    
     & 97.01
     & 15.26M
     & 591.65M
     
     \\
     VGG-S-split8
     
     & Flower102
     & 102 
     & 224$\x$224   
     & 8 
     & 85.66
     & 96.75
     & 7.64M 
     & 382.51M
  
     
     \\
  \bottomrule
\end{tabular}
}
\label{table:models-vision}
\vspace{-20pt}
\end{table}
\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>


==> tex/table-common-vision-fat-corl.tex <==
% SINGLE-COL TALBE
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%

%\renewcommand{\arraystretch}{0.88}
%\begin{table}

%\vspace{-10pt}
%\centering
%\caption{Results of split-fattened DNN models on Cifar10/100, and Flower102 datasets. For \texttt{[model\_name]-f[number]}, number represent the percentage of fattening, e.g., \texttt{*-f10} = 10\%.  }
\adjustbox{max width=\textwidth}{
\scriptsize
\vspace{5pt}
\begin{tabular}{c || c | c | c | c | c }
  \toprule
   \multirow{2}{*}{\textbf{Model Name}} 
      & \multirow{2}{*}{\textbf{Dataset}}
      & {\textbf{Top-1}}
      & {\textbf{Top-5}}
      & \textbf{\#}
      & \textbf{\# MAC} \\
   
            
      & 
      & {\textbf{Acc.}}
      & {\textbf{Acc.}}
      & \textbf{Param.}
      & \textbf{Opr.}\\
  
     \midrule 
     %-------------------------------------------
     \textbf{CifarNet}
     
     & \textbf{Cifar10} 
     & \textbf{83.41}
     & \textbf{98.86}
     & \textbf{797.97k}
     & \textbf{14.79M}
          
     \\
     CifarNet-split8
     
     & Cifar10
     & 76.70
     & 98.40
     & 104.6k
     & 5.22M
     
     \\
     CifarNet-split8-f10
     
     & Cifar10
     & 78.64
     & 98.67
     & 129.1k
     & 6.07M
     
     \\
     CifarNet-split8-f20
     
     & Cifar10
     & 79.65
     & 98.87
     & 156.16k
     & 6.95M
     
      \\
     CifarNet-split8-f30
     
     & Cifar10
     & 80.17
     & 98.90
     & 185.78k
     & 7.88M
     
     \\
     CifarNet-split8-f40
     
     & Cifar10
     & 81.10
     & 99.06
     & 240.61k
     & 9.85M
     
     
     \\
     \midrule
     
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Cifar100}
     & \textbf{50.33}
     & \textbf{75.26}
     & \textbf{76.15M}
     & \textbf{154.09M}
     
     \\
     VGG-S-split8
     
     & Cifar100
     & 48.48
     & 77.66
     & 9.54M
     & 21.42M
     
     \\
     VGG-S-split8-f10
     
     & Cifar100
     & 49.39
     & 77.73
     & 11.47M
     & 25.41M
     
     \\
     VGG-S-split8-f20
     
     & Cifar100
     & 49.78
     & 77.93
     & 13.58M
     & 29.74M
     
     \\
     VGG-S-split8-f30
     
     & Cifar100
     & 50.05
     & 77.90
     & 16.08M
     & 35.21M
     
     \\
     VGG-S-split8-f40
     
     & Cifar100
     & {\bf \color{black} 50.60}
     & 77.93
     & 18.74M
     & 40.86M

     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Flower102}
     & \textbf{88.14}
     & \textbf{97.02}
     & \textbf{60.79M}
     & \textbf{1.85G}
     
     
     \\
     VGG-S-split8
     
     & Flower102
     & 85.66
     & 96.75
     & 7.64M 
     & 382.51M
     
     
     \\
     VGG-S-split8-f10
     
     & Flower102
     & 87.92
     & 96.89
     & 9.14M
     & 437.06M
     
     \\
     VGG-S-split8-f20
     
     & Flower102
     & {\bf \color{black} 88.65}
     & 97.19
     & 10.57M
     & 487.47M
  
     \\
     VGG-S-split8-f30
     
     & Flower102
     & {\bf \color{black} 89.24}
     & 97.62
     & 12.7M
     & 589.12M

    \\
     VGG-S-split8-f40
     
     & Flower102
     & {\bf \color{black} 89.59}
     & 97.87
     & 14.74M
     & 660.05M
  
     
     \\
  \bottomrule
\end{tabular}
\label{table:models-vision-fat}
}
%\vspace{-15pt}
%\end{table}
%\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>



% FULL TALBE
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
%\renewcommand{\arraystretch}{1.0}
%\begin{table*}[h]
%\scriptsize
%\vspace{-0pt}
%\centering
%\caption{Results of split-fattened DNN models on Cifar10/100, and Flower102 datasets. fc: fully-connected, c: convolution, p: pooling, n: normalization, and d: dropout. For \texttt{[model\_name]-f[number]}, number represent the percentage of fattening, e.g., \texttt{*-f10} = 10\%.  }
%\vspace{5pt}
%\begin{tabular}{c || c | c | c | c | c | c | c | c | c }
%  \toprule
%   \multirow{2}{*}{Model Name} 
%      & \multirow{2}{*}{Dataset}
%      & \multirow{2}{*}{Classes}
%      & Input
%      & \multirow{2}{*}{Branches}
%      & Total Number
%      & {Top-1}
%      & {Top-5}
%      & Number of 
%      & Number of \\
%   
%            
%      & 
%      &
%      & Size
%      &
%      & of Layers
%      & {Accuracy}
%      & {Accuracy}
%      & Parameters
%      & MAC Operations\\
%  
%     \midrule 
%     %-------------------------------------------
%     CifarNet
%     
%     & Cifar10 
%     & 10
%     & 32$\x$32    
%     & 1
%     & 2fc-2c-2p-2n-1d
%     & 80.72
%     & 98.86
%     & 797.97k
%     & 14.79M
%          
%     \\
%     CifarNet-split8
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 76.70
%     & 98.40
%     & 104.6k
%     & 5.22M
%     
%     \\
%     CifarNet-split8-f10
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 78.64
%     & 98.67
%     & 129.1k
%     & 6.07M
%     
%     \\
%     CifarNet-split8-f20
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 79.65
%     & 98.87
%     & 156.16k
%     & 6.95M
%     
%      \\
%     CifarNet-split8-f30
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 80.17
%     & 98.90
%     & 185.78k
%     & 7.88M
%     
%     \\
%     CifarNet-split8-f40
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 81.10
%     & 99.06
%     & 240.61k
%     & 9.85M
%     
%     
%     \\
%     \midrule
%     
%     %-------------------------------------------
%     VGG-S
%     
%     & Cifar100
%     & 100
%     & 32$\x$32  
%     & 1
%     & 3fc-5c-2p-1n-2d 
%     & 50.33
%     & 75.26
%     & 76.15M
%     & 154.09M
%     
%     \\
%     VGG-S-split8
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 48.48
%     & 77.66
%     & 9.54M
%     & 21.42M
%     
%     \\
%     VGG-S-split8-f10
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 49.39
%     & 77.73
%     & 11.47M
%     & 25.41M
%     
%     \\
%     VGG-S-split8-f20
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 49.78
%     & 77.93
%     & 13.58M
%     & 29.74M
%     
%     \\
%     VGG-S-split8-f30
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 50.05
%     & 77.90
%     & 16.08M
%     & 35.21M
%     
%     \\
%     VGG-S-split8-f40
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 50.60
%     & 77.93
%     & 18.74M
%     & 40.86M
%
%     \\
%     \midrule
%     %-------------------------------------------
%     VGG-S
%     
%     & Flower102
%     & 102  
%     & 224$\x$224  
%     & 1
%     & 3fc-5c-3p-1n-2d 
%     & 88.14
%     & 97.02
%     & 60.79M
%     & 1.85G
%     
%     
%     \\
%     VGG-S-split8
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 85.66
%     & 96.75
%     & 7.64M 
%     & 382.51M
%     
%     
%     \\
%     VGG-S-split8-f10
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 87.92
%     & 96.89
%     & 9.14M
%     & 437.06M
%     
%     \\
%     VGG-S-split8-f20
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 88.65
%     & 97.19
%     & 10.57M
%     & 487.47M
%  
%     \\
%     VGG-S-split8-f30
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 89.24
%     & 97.62
%     & 12.7M
%     & 589.12M
%
%    \\
%     VGG-S-split8-f40
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 89.59
%     & 97.87
%     & 14.74M
%     & 660.05M
%  
%     
%     \\
%  \bottomrule
%\end{tabular}
%\label{table:models-vision-fat}
%\vspace{-10pt}
%\end{table*}
%\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>


==> tex/table-common-vision-fat.tex <==
% SINGLE-COL TALBE
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%


\renewcommand{\arraystretch}{0.88}
\begin{table}[h]
\scriptsize
\vspace{-10pt}
\centering
\caption{Results of split-fattened DNN models on Cifar10/100, and Flower102 datasets. For \texttt{[model\_name]-f[number]}, number represent the percentage of fattening, e.g., \texttt{*-f10} = 10\%.  }
\vspace{5pt}
\begin{tabular}{c || c | c | c | c | c }
  \toprule
   \multirow{2}{*}{\textbf{Model Name}} 
      & \multirow{2}{*}{\textbf{Dataset}}
      & {\textbf{Top-1}}
      & {\textbf{Top-5}}
      & \textbf{\#}
      & \textbf{\# MAC} \\
   
            
      & 
      & {\textbf{Acc.}}
      & {\textbf{Acc.}}
      & \textbf{Param.}
      & \textbf{Opr.}\\
  
     \midrule 
     %-------------------------------------------
     \textbf{CifarNet}
     
     & \textbf{Cifar10} 
     & \textbf{80.72}
     & \textbf{98.86}
     & \textbf{797.97k}
     & \textbf{14.79M}
          
     \\
     CifarNet-split8
     
     & Cifar10
     & 76.70
     & 98.40
     & 104.6k
     & 5.22M
     
     \\
     CifarNet-split8-f10
     
     & Cifar10
     & 78.64
     & 98.67
     & 129.1k
     & 6.07M
     
     \\
     CifarNet-split8-f20
     
     & Cifar10
     & 79.65
     & 98.87
     & 156.16k
     & 6.95M
     
      \\
     CifarNet-split8-f30
     
     & Cifar10
     & 80.17
     & 98.90
     & 185.78k
     & 7.88M
     
     \\
     CifarNet-split8-f40
     
     & Cifar10
     & {\bf \color{PineGreen} 81.10}
     & 99.06
     & 240.61k
     & 9.85M
     
     
     \\
     \midrule
     
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Cifar100}
     & \textbf{50.33}
     & \textbf{75.26}
     & \textbf{76.15M}
     & \textbf{154.09M}
     
     \\
     VGG-S-split8
     
     & Cifar100
     & 48.48
     & 77.66
     & 9.54M
     & 21.42M
     
     \\
     VGG-S-split8-f10
     
     & Cifar100
     & 49.39
     & 77.73
     & 11.47M
     & 25.41M
     
     \\
     VGG-S-split8-f20
     
     & Cifar100
     & 49.78
     & 77.93
     & 13.58M
     & 29.74M
     
     \\
     VGG-S-split8-f30
     
     & Cifar100
     & 50.05
     & 77.90
     & 16.08M
     & 35.21M
     
     \\
     VGG-S-split8-f40
     
     & Cifar100
     & {\bf \color{PineGreen} 50.60}
     & 77.93
     & 18.74M
     & 40.86M

     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG-S}
     
     & \textbf{Flower102}
     & \textbf{88.14}
     & \textbf{97.02}
     & \textbf{60.79M}
     & \textbf{1.85G}
     
     
     \\
     VGG-S-split8
     
     & Flower102
     & 85.66
     & 96.75
     & 7.64M 
     & 382.51M
     
     
     \\
     VGG-S-split8-f10
     
     & Flower102
     & 87.92
     & 96.89
     & 9.14M
     & 437.06M
     
     \\
     VGG-S-split8-f20
     
     & Flower102
     & {\bf \color{PineGreen} 88.65}
     & 97.19
     & 10.57M
     & 487.47M
  
     \\
     VGG-S-split8-f30
     
     & Flower102
     & {\bf \color{PineGreen} 89.24}
     & 97.62
     & 12.7M
     & 589.12M

    \\
     VGG-S-split8-f40
     
     & Flower102
     & {\bf \color{PineGreen} 89.59}
     & 97.87
     & 14.74M
     & 660.05M
  
     
     \\
  \bottomrule
\end{tabular}
\label{table:models-vision-fat}
\vspace{-10pt}
\end{table}
\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>



% FULL TALBE
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
%\renewcommand{\arraystretch}{1.0}
%\begin{table*}[h]
%\scriptsize
%\vspace{-0pt}
%\centering
%\caption{Results of split-fattened DNN models on Cifar10/100, and Flower102 datasets. fc: fully-connected, c: convolution, p: pooling, n: normalization, and d: dropout. For \texttt{[model\_name]-f[number]}, number represent the percentage of fattening, e.g., \texttt{*-f10} = 10\%.  }
%\vspace{5pt}
%\begin{tabular}{c || c | c | c | c | c | c | c | c | c }
%  \toprule
%   \multirow{2}{*}{Model Name} 
%      & \multirow{2}{*}{Dataset}
%      & \multirow{2}{*}{Classes}
%      & Input
%      & \multirow{2}{*}{Branches}
%      & Total Number
%      & {Top-1}
%      & {Top-5}
%      & Number of 
%      & Number of \\
%   
%            
%      & 
%      &
%      & Size
%      &
%      & of Layers
%      & {Accuracy}
%      & {Accuracy}
%      & Parameters
%      & MAC Operations\\
%  
%     \midrule 
%     %-------------------------------------------
%     CifarNet
%     
%     & Cifar10 
%     & 10
%     & 32$\x$32    
%     & 1
%     & 2fc-2c-2p-2n-1d
%     & 80.72
%     & 98.86
%     & 797.97k
%     & 14.79M
%          
%     \\
%     CifarNet-split8
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 76.70
%     & 98.40
%     & 104.6k
%     & 5.22M
%     
%     \\
%     CifarNet-split8-f10
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 78.64
%     & 98.67
%     & 129.1k
%     & 6.07M
%     
%     \\
%     CifarNet-split8-f20
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 79.65
%     & 98.87
%     & 156.16k
%     & 6.95M
%     
%      \\
%     CifarNet-split8-f30
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 80.17
%     & 98.90
%     & 185.78k
%     & 7.88M
%     
%     \\
%     CifarNet-split8-f40
%     
%     & Cifar10
%     & 10  
%     & 32$\x$32  
%     & 8
%     & 17fc-16c-16p-16n-8d
%     & 81.10
%     & 99.06
%     & 240.61k
%     & 9.85M
%     
%     
%     \\
%     \midrule
%     
%     %-------------------------------------------
%     VGG-S
%     
%     & Cifar100
%     & 100
%     & 32$\x$32  
%     & 1
%     & 3fc-5c-2p-1n-2d 
%     & 50.33
%     & 75.26
%     & 76.15M
%     & 154.09M
%     
%     \\
%     VGG-S-split8
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 48.48
%     & 77.66
%     & 9.54M
%     & 21.42M
%     
%     \\
%     VGG-S-split8-f10
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 49.39
%     & 77.73
%     & 11.47M
%     & 25.41M
%     
%     \\
%     VGG-S-split8-f20
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 49.78
%     & 77.93
%     & 13.58M
%     & 29.74M
%     
%     \\
%     VGG-S-split8-f30
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 50.05
%     & 77.90
%     & 16.08M
%     & 35.21M
%     
%     \\
%     VGG-S-split8-f40
%     
%     & Cifar100
%     & 100 
%     & 32$\x$32   
%     & 8 
%     & 17fc-40c-16p-8n-16d 
%     & 50.60
%     & 77.93
%     & 18.74M
%     & 40.86M
%
%     \\
%     \midrule
%     %-------------------------------------------
%     VGG-S
%     
%     & Flower102
%     & 102  
%     & 224$\x$224  
%     & 1
%     & 3fc-5c-3p-1n-2d 
%     & 88.14
%     & 97.02
%     & 60.79M
%     & 1.85G
%     
%     
%     \\
%     VGG-S-split8
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 85.66
%     & 96.75
%     & 7.64M 
%     & 382.51M
%     
%     
%     \\
%     VGG-S-split8-f10
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 87.92
%     & 96.89
%     & 9.14M
%     & 437.06M
%     
%     \\
%     VGG-S-split8-f20
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 88.65
%     & 97.19
%     & 10.57M
%     & 487.47M
%  
%     \\
%     VGG-S-split8-f30
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 89.24
%     & 97.62
%     & 12.7M
%     & 589.12M
%
%    \\
%     VGG-S-split8-f40
%     
%     & Flower102
%     & 102 
%     & 224$\x$224   
%     & 8 
%     & 17fc-40c-24p-8n-16d 
%     & 89.59
%     & 97.87
%     & 14.74M
%     & 660.05M
%  
%     
%     \\
%  \bottomrule
%\end{tabular}
%\label{table:models-vision-fat}
%\vspace{-10pt}
%\end{table*}
%\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>


==> tex/table-compare-intro-corl.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
\definecolor{bad}{rgb}{0.980, 0.878, 0.892}
\definecolor{ideal}{rgb}{0.85, 0.99, 0.852}
\definecolor{ideal2}{rgb}{0.592, 0.945, 0.533}
\definecolor{good}{rgb}{0.992, 0.984, 0.886}
\definecolor{grayMy}{rgb}{0.968, 0.968, 0.968}



\renewcommand{\arraystretch}{1.0}
\begin{table}[!t]
\scriptsize
\vspace{-0pt}
\centering
\caption{Distribution methods for the computation of inferencing in  DNNs.}
\vspace{-0pt}
\begin{tabular}{| c | c | c | c | c |}

      \hline
      \cellcolor{grayMy}
      & \cellcolor{grayMy}\textbf{Data} 
      & \cellcolor{grayMy} \textbf{Model}
      & \cellcolor{grayMy} 
      & \cellcolor{grayMy}  
      \\
      
      \cellcolor{grayMy}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \multirow{-2}{*}{\cellcolor{grayMy}\textbf{Target}}
      & \multirow{-2}{*}{\cellcolor{grayMy} \textbf{Proposed Models}}
      \\
      \hline
      
      %------------
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Memory}}
      & \cellcolor{bad}  
      & \cellcolor{ideal} 
      & \cellcolor{ideal}  
      & \cellcolor{ideal2} 
      \\
      
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad}DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Communication}}
      & \cellcolor{ideal} 
      & \cellcolor{bad}  Intermediates
      & \cellcolor{ideal} 
      & \cellcolor{good} 
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Inference}}
      & \multirow{-2}{*}{\cellcolor{ideal}$\text{IN}/\text{OUT}$}
      & \cellcolor{bad} $+ \text{IN}/\text{OUT}$
      & \multirow{-2}{*}{\cellcolor{ideal} $\text{IN}/\text{OUT}$}
      & \multirow{-2}{*}{\cellcolor{good} $\approx\text{IN}/\text{OUT}$}
      \\
      
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Computation}}
      & \cellcolor{bad}
      & \cellcolor{ideal}
      & \cellcolor{ideal}
      & \cellcolor{ideal2}
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad} DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      
      \hline
      
      %------------
%       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Features or}}
%       & \cellcolor{grayMy} Requires Multiple
%       & \cellcolor{grayMy} Relies on
%       & \cellcolor{grayMy}
%       & \cellcolor{grayMy}
%       \\
%      
%      
%      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Barriers}}
%      & \cellcolor{grayMy} Requests
%      & \cellcolor{grayMy} Fast Communication
%      & \cellcolor{grayMy}
%      & \cellcolor{grayMy}
%      \\
%      \hline
  
     %-------------------------------------------
     
  
\end{tabular}
\label{table:compare-intro}
\vspace{-20pt}
\end{table}
\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>

==> tex/table-compare-intro-micro-extended.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
\definecolor{bad}{rgb}{0.980, 0.878, 0.892}
\definecolor{ideal}{rgb}{0.85, 0.99, 0.852}
\definecolor{ideal2}{rgb}{0.592, 0.945, 0.533}
\definecolor{good}{rgb}{0.992, 0.984, 0.886}
\definecolor{grayMy}{rgb}{0.968, 0.968, 0.968}


\renewcommand{\arraystretch}{0.90}
\begin{table}[b]
\centering

\begin{adjustbox}{max width=\columnwidth}



\begin{threeparttable}
\centering  

\vspace{-4pt}
\caption{Methods for distributing inference computations. \vspace{-5pt}}



\scriptsize

\begin{tabular}{| c | c | c | c | c |}

      \hline
      \cellcolor{grayMy}
      & \cellcolor{grayMy}\textbf{Data} 
      & \cellcolor{grayMy} \textbf{Model}
      & \cellcolor{grayMy} 
      & \cellcolor{grayMy}  
      \\
      
      \cellcolor{grayMy}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \multirow{-2}{*}{\cellcolor{grayMy}\textbf{Target}}
      & \multirow{-2}{*}{\cellcolor{grayMy} \textbf{LCP}}
      \\
      \hline
      
      %------------
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Memory}}
      & \cellcolor{bad}  
      & \cellcolor{ideal} 
      & \cellcolor{ideal}  
      & \cellcolor{ideal2} 
      \\
      
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad}DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Communication}}
      & \cellcolor{ideal} 
      & \cellcolor{bad}  Intermediates
      & \cellcolor{ideal} 
      & \cellcolor{good} 
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Inference}}
      & \multirow{-2}{*}{\cellcolor{ideal}$\text{IN}/\text{OUT}$}
      & \cellcolor{bad} $+ \text{IN}/\text{OUT}$
      & \multirow{-2}{*}{\cellcolor{ideal} $\text{IN}/\text{OUT}$}
      & \multirow{-2}{*}{\cellcolor{good} $\approx\text{IN}/\text{OUT}$}
      \\
      
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Computation}}
      & \cellcolor{bad}
      & \cellcolor{ideal}
      & \cellcolor{ideal}
      & \cellcolor{ideal2}
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad} DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      
      \hline
  
     %-------------------------------------------
     
  
\end{tabular}

\begin{tablenotes}[flushright]
    \item[] \hspace{50pt}DNN: Metrics associated with the entire model; $n$: Number of devices.
\end{tablenotes}
  
  
\label{table:compare-intro}

\end{threeparttable}

\end{adjustbox}

\vspace{-5pt}



\end{table}
\renewcommand{\arraystretch}{1}

%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>

==> tex/table-compare-intro.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
\definecolor{bad}{rgb}{0.980, 0.878, 0.892}
\definecolor{ideal}{rgb}{0.85, 0.99, 0.852}
\definecolor{ideal2}{rgb}{0.592, 0.945, 0.533}
\definecolor{good}{rgb}{0.992, 0.984, 0.886}
\definecolor{grayMy}{rgb}{0.968, 0.968, 0.968}



\renewcommand{\arraystretch}{1.0}
\begin{table}[!t]
\scriptsize
\vspace{-0pt}
\centering
\caption{Distribution methods for the computation of inferencing in  DNNs.}
\vspace{-0pt}
\begin{tabular}{| c | c | c | c | c |}

      \hline
      \cellcolor{grayMy}
      & \cellcolor{grayMy}\textbf{Data} 
      & \cellcolor{grayMy} \textbf{Model}
      & \cellcolor{grayMy} 
      & \cellcolor{grayMy}  
      \\
      
      \cellcolor{grayMy}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \cellcolor{grayMy} \textbf{Parallelism}
      & \multirow{-2}{*}{\cellcolor{grayMy}\textbf{Target}}
      & \multirow{-2}{*}{\cellcolor{grayMy} \textbf{Proposed Models}}
      \\
      \hline
      
      %------------
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Memory}}
      & \cellcolor{bad}  
      & \cellcolor{ideal} 
      & \cellcolor{ideal}  
      & \cellcolor{ideal2} 
      \\
      
      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad}DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Communication}}
      & \cellcolor{ideal} 
      & \cellcolor{bad}  Intermediates
      & \cellcolor{ideal} 
      & \cellcolor{good} 
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Inference}}
      & \multirow{-2}{*}{\cellcolor{ideal}$\text{IN}/\text{OUT}$}
      & \cellcolor{bad} $+ \text{IN}/\text{OUT}$
      & \multirow{-2}{*}{\cellcolor{ideal} $\text{IN}/\text{OUT}$}
      & \multirow{-2}{*}{\cellcolor{good} $\approx\text{IN}/\text{OUT}$}
      \\
      
      \hline
      
      %------------
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Computation}}
      & \cellcolor{bad}
      & \cellcolor{ideal}
      & \cellcolor{ideal}
      & \cellcolor{ideal2}
      \\
      
       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Per Device}}
      & \multirow{-2}{*}{\cellcolor{bad} DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal} $\frac{1}{n}$DNN}
      & \multirow{-2}{*}{\cellcolor{ideal2} $\leq \frac{1}{n}$DNN}
      \\
      
      \hline
      
      %------------
%       \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Features or}}
%       & \cellcolor{grayMy} Requires Multiple
%       & \cellcolor{grayMy} Relies on
%       & \cellcolor{grayMy}
%       & \cellcolor{grayMy}
%       \\
%      
%      
%      \multicolumn{1}{|c|}{\cellcolor{grayMy} \textbf{Barriers}}
%      & \cellcolor{grayMy} Requests
%      & \cellcolor{grayMy} Fast Communication
%      & \cellcolor{grayMy}
%      & \cellcolor{grayMy}
%      \\
%      \hline
  
     %-------------------------------------------
     
  
\end{tabular}
\label{table:compare-intro}
\vspace{-20pt}
\end{table}
\renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>

==> tex/table-image-net-fat-corl.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
\begin{wraptable}{r}{0.60\textwidth}

\renewcommand{\arraystretch}{0.88}
%\begin{table}[!t]
\scriptsize
\vspace{0pt}
\centering
\caption{Results of split-fattened DNN models on ImageNet datasets. For \texttt{[model\_name]-f[number]}, number represent the percentage of fattening.}
\label{table:models-imagenet-fat}
\vspace{5pt}
\begin{tabular}{c || c | c | c | c | c }
  \toprule
   \multirow{2}{*}{\textbf{Model Name}} 
      & \multirow{2}{*}{\textbf{Dataset}}
      & {\textbf{Top-1}}
      & {\textbf{Top-5}}
      & \textbf{\#} 
      & \textbf{\# MAC} \\
   
            
      & 
      & {\textbf{Acc.}}
      & {\textbf{Acc.}}
      & \textbf{Param.}
      & \textbf{MAC Opr.}\\
      \midrule 
  
     %-------------------------------------------
     \textbf{AlexNet}
     
     & \textbf{ImageNet}
     & \textbf{57.02}
     & \textbf{80.32}
     & \textbf{50.3M}
     & \textbf{678.97M}
     
     \\
     AlexNet-split8
     
     & ImageNet
     & 49.03
     & 73.10
     & 6.32M 
     & 145.37M
     
     \\
     AlexNet-split8-f10
     
     & ImageNet
     & 51.81
     & 74.20
     & 7.56M 
     & 170.1M

     \\
     AlexNet-split8-f20
     
     & ImageNet
     & 52.65
     & 74.92
     & 8.92M
     & 197.94M
     
     \\
     AlexNet-split8-f30
     
     & ImageNet
     & 53.45
     & 75.32
     & 10.52M  
     & 213.04M
     
     \\
     AlexNet-split8-f40
     
     & ImageNet
     & {\bf \color{black} 54.68}
     & 77.06
     & 12.11M
     & 244M

     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG16}
     
     & \textbf{ImageNet}
     & \textbf{70.48}
     & \textbf{90.02}
     & \textbf{138.36M}
     & \textbf{15.47G}
     
     \\
     VGG16-split8
     
     & ImageNet
     & 58.67
     & 81.54
     & 7.64M
     & 2.01G
     
     \\
     VGG16-split8-f10
     
     & ImageNet
     & 60.02
     & 84.12
     & 20.77M
     & 2.44G
     
    \\
     VGG16-split8-f20
     
     & ImageNet
     & 61.92
     & 84.95
     & 24.83M
     & 2.89G
     
     \\
     VGG16-split8-f30
     
     & ImageNet
     & 64.22
     & 87.54
     & 29.01M
     & 3.35G
     
     \\
     VGG16-split8-f40
     
     & ImageNet
     & {\bf \color{black}67.24}
     & 89.23
     & 33.78M
     & 3.87G
  
     
     \\
  \bottomrule
\end{tabular}

\vspace{-8pt}
%\end{table}
\renewcommand{\arraystretch}{1}

\end{wraptable}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>


==> tex/table-image-net.tex <==
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
%
%
%
%% FULL TABLE MICRO
% \renewcommand{\arraystretch}{0.88}
% \begin{table*}[!t]
% \scriptsize
% \vspace{-0pt}
% \centering
% \caption{Results of split-only DNN models on ImageNet datasets. fc: fully-connected, c: convolution, p: pooling, n: normalization, and d: dropout.}
% \vspace{5pt}
% \begin{tabular}{c || c | c | c | c | c | c | c | c | c }
%   \toprule
%   \multirow{2}{*}{\textbf{Model Name}} 
%       & \multirow{2}{*}{\textbf{Dataset}}
%       & \multirow{2}{*}{\textbf{Classes}}
%       & \textbf{Input}
%       & \multirow{2}{*}{\textbf{Branches}}
%       & \textbf{Total Number}
%       & {\textbf{Top-1}}
%       & {\textbf{Top-5}}
%       & \textbf{Number of} 
%       & \textbf{Number of} \\
   
            
%       & 
%       &
%       & \textbf{Size}
%       &
%       & \textbf{of Layers}
%       & {\textbf{Accuracy}}
%       & {\textbf{Accuracy}}
%       & \textbf{Parameters}
%       & \textbf{MAC Operations}\\
%       \midrule 
  
%      %-------------------------------------------
%      \textbf{AlexNet}
     
%      & \textbf{ImageNet}
%      & \textbf{1000}
%      & \textbf{224$\x$224}  
%      & \textbf{1}
%      & \textbf{7c-3p-2n-2d}
%      & \textbf{57.02}
%      & \textbf{80.32}
%      & \textbf{50.3M}
%      & \textbf{678.97M}
     
%      \\
%      AlexNet-split2
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 2
%      & 13c-6p-4n-4d 
%      & 53.27
%      & 76.97
%      & 25.17M
%      & 374.06M
     
%      \\
%      AlexNet-split4
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 4
%      & 25c-12p-8n-8d 
%      & 49.88
%      & 72.85
%      & 12.6M
%      & 221.6M
     
%      \\
%      AlexNet-split8
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 8
%      & 49c-24p-16n-16d  
%      & 49.03
%      & 73.10
%      & 6.32M 
%      & 145.37M

%      \\
%      \midrule
%      %-------------------------------------------
%      \textbf{VGG16}
     
%      & \textbf{ImageNet}
%      & \textbf{1000}
%      & \textbf{224$\x$224}  
%      & \textbf{1}
%      & \textbf{16c-5p-2d} 
%      & \textbf{70.48}
%      & \textbf{90.02}
%      & \textbf{138.36M}
%      & \textbf{15.47G}
     
%      \\
%      VGG16-split2
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 2
%      & 31c-10p-4d  
%      & 65.79
%      & 87.84
%      & 69.19M
%      & 7.78G
     
%      \\
%      VGG16-split4
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 4
%      & 61c-20p-8d 
%      & 61.01
%      & 83.02
%      & 34.6M
%      & 3.93G
     
%      \\
%      VGG16-split8
     
%      & ImageNet
%      & 1000
%      & 224$\x$224  
%      & 8
%      & 121c-40p-16d 
%      & 58.67
%      & 81.54
%      & 17.31M
%      & 2.01G
  
     
%      \\
%   \bottomrule
% \end{tabular}
% \label{table:models-imagenet}
% \vspace{-0pt}
% \end{table*}
% \renewcommand{\arraystretch}{1}
%
%
%
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>
% >>>>>>>>>>>>>>>>>>>>>>>>>>


\renewcommand{\arraystretch}{0.88}
\begin{table}[!t]
\scriptsize
\vspace{-0pt}
\centering
\caption{Specification of ImageNet Baseline DNN models.}
\vspace{5pt}
\begin{tabular}{c || c | c | c | c | c }
  \toprule
   \multirow{2}{*}{\textbf{Model Name}} 
      & \multirow{2}{*}{\textbf{Dataset}}
      & {\textbf{Top-1}}
      & {\textbf{Top-5}}
      & \textbf{\#} 
      & \textbf{\# MAC} \\
   
            
      & 
      & {\textbf{Acc.}}
      & {\textbf{Acc.}}
      & \textbf{Param.}
      & \textbf{Opr.}\\
      \midrule 
  
     %-------------------------------------------
     \textbf{AlexNet}
     
     & \textbf{ImageNet}
     & \textbf{57.02}
     & \textbf{80.32}
     & \textbf{50.3M}
     & \textbf{678.97M}
     
    %  \\
    %  AlexNet-split2
     
    %  & ImageNet
    %  & 53.27
    %  & 76.97
    %  & 25.17M
    %  & 374.06M
     
    %  \\
    %  AlexNet-split4
     
    %  & ImageNet
    %  & 49.88
    %  & 72.85
    %  & 12.6M
    %  & 221.6M
     
    %  \\
    %  AlexNet-split8
     
    %  & ImageNet
    %  & 49.03
    %  & 73.10
    %  & 6.32M 
    %  & 145.37M

     \\
     \midrule
     %-------------------------------------------
     \textbf{VGG16}
     
     & \textbf{ImageNet}
     & \textbf{70.48}
     & \textbf{90.02}
     & \textbf{138.36M}
     & \textbf{15.47G}
     
     \\
    %  VGG16-split2
     
    %  & ImageNet
    %  & 65.79
    %  & 87.84
    %  & 69.19M
    %  & 7.78G
     
    %  \\
    %  VGG16-split4
     
    %  & ImageNet
    %  & 61.01
    %  & 83.02
    %  & 34.6M
    %  & 3.93G
     
    %  \\
    %  VGG16-split8
     
    %  & ImageNet
    %  & 58.67
    %  & 81.54
    %  & 17.31M
    %  & 2.01G
  
     
    %  \\
  \bottomrule
\end{tabular}
\label{table:models-imagenet}
\vspace{-0pt}
\end{table}
\renewcommand{\arraystretch}{1}

==> tex/table-split-cascaded-model.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\renewcommand{\arraystretch}{1.3}
\scriptsize
\vspace{0pt}
\centering
\caption{Results of Split-Cascaded Model. \textbf{Cascade} represents the cascade classifier, and \textbf{Branch} represents the individual branch classifier. Number represents how model is split. E.g. $2 * \frac{1}{4} + \frac{1}{2}$ stands for the model is split into $2$ branch with $\frac{1}{4}$ of original size and $1$ branch with $\frac{1}{2}$ size.}
\vspace{5pt}
\begin{tabular}{ c || c | c | c }
    \toprule
    \multirow{2}{*}{\textbf{Model Name}}
    & \textbf{Top-1}
    & \textbf{\# of}
    & \textbf{\# Mac}
    \\
    
    
    & \textbf{Acc.}
    & \textbf{Param}
    & \textbf{Opr.}
    \\
    \midrule
                            
    CifarNet
    & 83.41
    & 799K
    & 14.79M
    \\
    \midrule
                            
    Cascade $2 * \frac{1}{2}$
    & 81.47
    & 748K
    & 14.79M
    \\
    
    Cascade $4 * \frac{1}{4}$
    & 81.53
    & 723K
    & 14.79M
    \\
    
    Cascade $\frac{1}{4} + \frac{3}{4}$
    & 82.16
    & 761K
    & 14.79M
    \\
    
    Cascade $2 * \frac{1}{4} + \frac{1}{2}$
    & 81.32
    & 735K
    & 14.79M
    \\
    
    Cascade $8 * \frac{1}{8}$
    & 79.73
    & 710K
    & 14.79M
    \\
    
    Cascade $\frac{1}{8} + \frac{7}{8}$
    & 82.64
    & 777K
    & 14.79M
    \\
    \midrule
                            
    Branch $\frac{1}{8}$
    & 57.30
    & 13K
    & 653.23K
    \\
                            
    Branch $\frac{1}{4}$
    & 70.92 
    & 52K
    & 1.65M
    \\
    
    Branch $\frac{1}{2}$
    & 77.47
    & 202K
    & 4.66M
    \\
    
    Branch $\frac{3}{4}$
    & 80.80
    & 451K
    & 9.04M
    \\
    
    Branch $\frac{7}{8}$
    & 82.17
    & 613K
    & 11.74M
    \\
    \bottomrule
\end{tabular}
\label{table:split-cascaded-model}
\renewcommand{\arraystretch}{1}
\end{wraptable}
